Data-Driven Random Access Optimization in Multi-Cell IoT Networks with NOMA

Non-orthogonal multiple access (NOMA) is a key technology to enable massive machine type communications (mMTC) in 5G networks and beyond. In this paper, NOMA is applied to improve the random access efficiency in high-density spatially-distributed multi-cell wireless IoT networks, where IoT devices contend for accessing the shared wireless channel using an adaptive p-persistent slotted Aloha protocol. To enable a capacity-optimal network, a novel formulation of random channel access management is proposed, in which the transmission probability of each IoT device is tuned to maximize the geometric mean of users' expected capacity. It is shown that the network optimization objective is high dimensional and mathematically intractable, yet it admits favourable mathematical properties that enable the design of efficient data-driven algorithmic solutions which do not require a priori knowledge of the channel model or network topology. A centralized model-based algorithm and a scalable distributed model-free algorithm, are proposed to optimally tune the transmission probabilities of IoT devices and attain the maximum capacity. The convergence of the proposed algorithms to the optimal solution is further established based on convex optimization and game-theoretic analysis. Extensive simulations demonstrate the merits of the novel formulation and the efficacy of the proposed algorithms.

==> bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figs/sammy.jpg}}]%
{Sami Khairy} (S’16) received the B.S. degree in Computer Engineering from the University of Jordan, Amman, Jordan, in 2014 and the M.S. degree in Electrical Engineering from Illinois Institute of Technology, Chicago, IL, USA, in 2016. He is currently working towards the Ph.D. degree in Electrical Engineering at Illinois Institute of Technology. His research interests span the broad areas of analysis and protocol design for next generation wireless networks, AI powered wireless networks resource management, reinforcement learning, statistical learning, and statistical signal processing. He received a Fulbright Predoctoral Scholarship from JACEE and the U.S. Department of State in 2015, and the Starr/Fieldhouse Research Fellowship from IIT in 2019. He is an IEEE student member and a member of IEEE ComSoc and IEEE HKN.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figs/prasanna.png}}]%
{Prasanna Balaprakash} is a computer scientist at the Mathematics and Computer Science Division with a joint appointment in the Leadership Computing Facility at Argonne National Laboratory. His research interests span the areas of artificial intelligence, machine learning, optimization, and high-performance computing. Currently, his research focuses on the development of scalable, data-efficient machine learning methods for scientific applications. He is a recipient of U.S. Department of Energy 2018 Early Career Award. Prior to Argonne, he worked as a Chief Technology Officer at Mentis Sprl, a machine learning startup in Brussels, Belgium. He received his PhD from CoDE-IRIDIA (AI Lab), Université Libre de Bruxelles, Brussels, Belgium, where he was a recipient of Marie Curie and F.R.S-FNRS Aspirant fellowships.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figs/lin.png}}]
{Lin X. Cai} (S’09–M’11–SM’19) received the M.A.Sc. and Ph.D. degrees in Electrical and Computer Engineering from the University of Waterloo, Waterloo, Canada, in 2005 and 2010, respectively. She is currently an Associate Professor with the Department of Electrical and Computer Engineering, Illinois Institute of Technology, Chicago, Illinois, USA. Her research interests include green communication and networking, intelligent radio resource management, and wireless Internet of Things. She received a Postdoctoral Fellowship Award from the Natural Sciences and Engineering Research Council of Canada (NSERC) in 2010, a Best Paper Award from the IEEE Globecom 2011, an NSF Career Award in 2016, and the IIT Sigma Xi Research Award in the Junior Faculty Division in 2019. She is an Associated Editor of IEEE Transaction on Wireless Communications, IEEE Network Magazine, and a co-chair for IEEE conferences.  
\end{IEEEbiography}


\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figs/poor-v.jpg}}]
{H. Vincent Poor} (S’72, M’77, SM’82, F’87) received the Ph.D. degree in EECS from Princeton
University in 1977. From 1977 until 1990, he was
on the faculty of the University of Illinois at Urbana-Champaign. Since 1990 he has been on the faculty
at Princeton, where he is the Michael Henry Strater
University Professor of Electrical Engineering and
Dean of the School of Engineering and Applied Science. Dr. Poor’s research interests are in the areas of
stochastic analysis, statistical signal processing and
their applications in wireless networks and related
fields. Among his publications in these areas is the recent book MIMO Wireless Communications (Cambridge University Press, 2007).
Dr. Poor is a member of the National Academy of Engineering, a Fellow of the American Academy of Arts and Sciences, and a former Guggenheim Fellow. He is also a Fellow of the Institute of Mathematical Statistics, the
Optical Society of America, and other organizations. In 1990, he served as President of the IEEE Information Theory Society, and in 2004-07 he served as the Editor-in-Chief of the IEEE IEEE TRANSACTIONS ON INFORMATION THEORY. He is the recipient of the 2005 IEEE Education Medal.
\end{IEEEbiography}

\begin{comment}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figs/cheng.png}}]
{Yu Cheng} (S’01–M’04–SM’09) received the B.E. and M.E. degrees in electronic engineering from Tsinghua University, Beijing, China, in 1995 and 1998, respectively, and the Ph.D. degree in electrical and computer engineering from the University of Waterloo, Waterloo, ON, Canada, in 2003. He is currently a Full Professor with the Department of Electrical and Computer Engineering, Illinois Institute of Technology, Chicago, IL, USA. His current research interests include wireless network performance analysis, network security, big data, cloud computing, and machine learning. Dr. Cheng was a recipient of the Best Paper Award at QShine 2007, the IEEE ICC 2011, the Runner-Up Best Paper Award at ACM MobiHoc 2014, the National Science Foundation CAREER Award in 2011, and the IIT Sigma Xi Research Award in the Junior Faculty Division in 2013. He has served as several Symposium Co-Chairs for IEEE ICC and IEEE GLOBECOM, and the Technical Program Committee Co-Chair for WASA 2011 and ICNC 2015. He was a founding Vice Chair of the IEEE ComSoc Technical Subcommittee on Green Communications and Computing. He was an IEEE ComSoc Distinguished Lecturer from 2016 to 2017. He is an Associate Editor for the IEEE Transactions on Vehicular Technology, IEEE Internet of Things Journal, and IEEE Wireless Communications.
\end{IEEEbiography}
\end{comment}
